Language Scaling for Universal Suggested Replies Model

We consider the problem of scaling automated suggested replies for Outlook email system to multiple languages. Faced with increased compute requirements and low resources for language expansion, we build a single universal model for improving the quality and reducing run-time costs of our production system. However, restricted data movement across regional centers prevents joint training across languages. To this end, we propose a multi-task continual learning framework, with auxiliary tasks and language adapters to learn universal language representation across regions. The experimental results show positive cross-lingual transfer across languages while reducing catastrophic forgetting across regions. Our online results on real user traffic show significant gains in CTR and characters saved, as well as 65% training cost reduction compared with per-language models. As a consequence, we have scaled the feature in multiple languages including low-resource markets.

==> review_suggestions.tex <==
Review 1:
- Lacks an analysis of failing cases of the system, and the possible harm of such failures
- focuses a small set of languages, most of which are high-resource European languages, which is not ideal for investigating multilingual approaches.

- It should be beneficial to further address the order of the application of continual learning and to see how different orders (e.g., across different language families) impact the performance of the final system


Review 2:
"Compared with per-language separate model building, around 65% training and performance improvement cost" - can the authors provide some details on how they reached the 65%, what proportion is infrastructure cost and what proportion is engineering cost ?

Minor comments:

Abstract: CTR is not explained

Section 4: During prediction, we use top N1 = 30, N2 = 3 for all the languages. What does this mean ?


Review 3:
One aspect I would love to see described more is the data itself; there is no discussion of:
- the length of the emails in the m-r pairs; was the data filtered at all to focus on relatively short emails that have straightforward responses?
- whether the domains of these emails were personal, business, or a mixture
- what exactly was the source of these emails ?  the authors simply call this "commercial email data" (in terms of the ethics questions, this is what left me wondering)
- what is the size of the curated response set?


Also, while the authors cite all of the work they build on, there is no discussion of other SR approaches for comparison as Related Work.  There are citations in the first paragraph of the Introduction, but no explicit comparison to their approaches and results


==> tex/related_work.tex <==
%An overview of existing modeling techniques related with suggested replies / search relevance problems, and cross-lingual model transfer on relevance problems, and other scenarios.

% [Will be merged into Intro Section, but hold it later.]

%I. Intelligent Conversation
% Various of Intelligent conversation systems are playing important roles in many scenarios. Recent examples include open-domain social chatbot\cite{zhou2020design}, task-oriented conversational agents assisting users to complete tasks in specific domains or offering valuable cognitive and emotional assistance \cite{Henderson2019b,fadhil2019designing,xu2017new,okuda2018ai,kopp2018conversational}, and social applications providing users with short, relevant and direct reply candidates such as Gmail, Outlook and  LinkedIn and Microsoft Teams\cite{Kannan2016,HendersonASSLGK17,shang2015neural}, known as Smart Reply or Suggested Reply(SR).

%II Seq2Seq vs IR-Matching
% The SR feature is similar to intelligent conversation systems such as open-domain social chat-bots and task-oriented conversational agents, \cite{zhou2020design, Henderson2019b,fadhil2019designing,xu2017new,okuda2018ai,kopp2018conversational}. In terms of usage, SR is closer to the latter, in that it assists users to complete a reply, instead of continuing an open-ended dialog. 

% S2S-based model could be traced back to \cite{ritter2011data}, a data-driven generative approach to generating responses to Twitter status posts, based on phrase-based SMT. \cite{Kannan2016} expends it to NMT \cite{sutskever2014sequence} using LSTM, predicting full responses in a limited candidate set. \cite{madotto2018mem2seq,ghazvininejad2018knowledge} further condition responses on external knowledge base. 

% SR can be modeled either as sequence-to-sequence (S2S) generation process, or in Information Retrieval (IR) fashion. IR-based model is more popular in production systems \cite{guo2020deep, henderson2017efficient, Deb2019DiversifyingRS}, since it allows careful selection and ranking of responses allowing better control of the feature. \cite{henderson2017efficient} achieves comparable performance as \cite{Kannan2016} at a smaller fraction of the computational requirements and latency. \cite{Deb2019DiversifyingRS} diversifies responses by formulating the model as a generative latent variable model with Conditional Variational Auto-Encoder.

% % II.B Joint Encoder vs Dual Encoder
% The matching score between message and reply candidates can be computed with either Joint Scoring or Dual-Encoder Matching architecture.

% %Joint Encoder
% Like \cite{devlin2018bert}, Joint Encoder encodes the combinations of input message and each response candidate, then learn their matching score directly. While it is beneficial to better interaction within the pair, the latency issue is unavoidable when it comes with tens of thousands of candidate replies.

%Dual Encoder
% Dual Encoder, two independent encoders with same architecture, encodes messages and replies independently into a shared space.\cite{swanson2019building,gillick2018end} It allows the fixed set of responses to be pre-encoded offline. At inference time, only input message need to be encoded, then the matching score of each M-R pair is computed by cosine distance. 

% In consideration of higher inference efficiency and better quality control, we choose a standard IR-based matching architecture to model the relevance between an input message and the responses from a fixed list.

%IV. Cross-lingual Semantic Representation
% Monolingual self-supervised representation learning captures significant underlying semantic information. 

% \cite{devlin2018bert,liu2019roberta,yang2019xlnet} demonstrate that there are considerable improvements by fine-tuning transformer-based pretrained models on specific tasks which has recently become a standardized process of state-of-the-art results. For our universal model, we fine-tune a XLM-R \cite{conneau2019unsupervised} like multi-lingual encoder. 

% Several papers have enhanced their cross-lingual, multi-lingual, and zero-shot scenarios, by leveraging parallel data and different pre-training tasks \cite{devlin2018bert,conneau2019unsupervised,chi2020infoxlm}. Such universal representations has led to enormous progress of standard benchmarks \cite{liang2020xglue,conneau2018xnli} and spawned several industrial applications such as language-agnostic identification on offensive language \cite{ranasinghe2020multilingual} and discourse classification \cite{gencoglu2020large} on social media.

